Rotations and Interpretability of Word Embeddings: the Case of the Russian Language

Consider a continuous word embedding model. Usually, the cosines between word vectors are used as a measure of similarity of words. These cosines do not change under orthogonal transformations of the embedding space. We demonstrate that, using some canonical orthogonal transformations from SVD, it is possible both to increase the meaning of some components and to make the components more stable under re-learning. We study the interpretability of components for publicly available models for the Russian language (RusVectores, fastText, RDT).

==> table_rusvectores_ruwikiruscorpora_ndim50.head100K.top15.tex <==
\selectlanguage{russian}
\centering
\footnotesize
\begin{tabular}{|m{0.5cm} | p{11.5cm}|}
\hline
\begin{center}1\end{center} &
\begin{tabular}{p{11.25cm}}
подумать{\tiny verb} глядеть{\tiny verb} молчать{\tiny verb} удивляться{\tiny verb} вздыхать{\tiny verb} нынче{\tiny adv} соображать{\tiny verb} поглядеть{\tiny verb} наверно{\tiny adv} постоять{\tiny verb} трогать{\tiny verb} деваться{\tiny verb} твердить{\tiny verb} видать{\tiny adv} подуматься{\tiny verb}
\\
\hline
год{\tiny noun} первый{\tiny adj} начало{\tiny noun} период{\tiny noun} серия{\tiny noun} ранее{\tiny adv} последующий{\tiny adj} первоначально{\tiny adv} изначально{\tiny adv};
также{\tiny adv} сша{\tiny noun} качество{\tiny noun} частность{\tiny noun} британский{\tiny adj} великобритания{\tiny noun}
\\
\end{tabular}\\
\hline
\begin{center}2\end{center} &
\begin{tabular}{p{11.25cm}}
россия{\tiny noun} государственный{\tiny adj} установление{\tiny noun} содействовать{\tiny verb};
признавать{\tiny verb} ограничиваться{\tiny verb} возлагать{\tiny verb} обусловливаться{\tiny verb} осуществимый{\tiny adj} диктоваться{\tiny verb} уяснение{\tiny noun} подготовление{\tiny noun}
\\
\hline
бейра::алта{\tiny noun} дора::литорал{\tiny noun} бейра::литорал{\tiny noun} эштремадура{\tiny noun} доур{\tiny noun} тамега{\tiny noun} минью::лима{\tiny noun} климат::полуконтинентальный{\tiny noun} бейра::байша{\tiny noun} vcc::pgc{\tiny noun} алта::алентеж{\tiny noun} чуровский{\tiny adj} байша::воуга{\tiny noun} оэшт{\tiny noun} байша::мондега{\tiny noun}
\\
\end{tabular}\\
\hline
\begin{center}3\end{center} &
\begin{tabular}{p{11.25cm}}
отец{\tiny noun} сын{\tiny noun} брат{\tiny noun} дочь{\tiny noun} замуж{\tiny adv} племянник{\tiny noun} зять{\tiny noun} настояние{\tiny noun};
александр{\tiny noun} николай{\tiny noun} михаил{\tiny noun} павел{\tiny noun} константин{\tiny noun} георгий{\tiny noun}
\\
\hline
проволочный{\tiny adj} сетчатый{\tiny adj} ленточный{\tiny adj} покровный{\tiny adj} ячеистый{\tiny adj} гофрированный{\tiny adj} перфорированный{\tiny adj} уплотненный{\tiny adj} гофрировать{\tiny verb} смазываться{\tiny verb} слоеный{\tiny adj} многокамерный{\tiny adj};
прессованный{\tiny adj} упаковываться{\tiny verb}
\\
\end{tabular}\\
\hline
\begin{center}4\end{center} &
\begin{tabular}{p{11.25cm}}
район{\tiny noun} село{\tiny noun} участок{\tiny noun} пос{\tiny noun} березовка{\tiny noun} оскол{\tiny noun} елшанка{\tiny noun} белоярский{\tiny adj};
грязнов{\tiny noun} елизаров{\tiny noun} позняк{\tiny noun} реут{\tiny noun} куркин{\tiny noun} полуэктов{\tiny noun} чиркин{\tiny noun}
\\
\hline
сделать{\tiny verb} приносить{\tiny verb} затмевать{\tiny verb};
признаваться{\tiny verb} соблазнять{\tiny verb} разочаровывать{\tiny verb} шокировать{\tiny verb} разочаровываться{\tiny verb} помешанный{\tiny adj};
вдохновлять{\tiny verb} восхищаться{\tiny verb} восхищать{\tiny verb} вдохновляться{\tiny verb}
\\
\end{tabular}\\
\hline
\begin{center}5\end{center} &
\begin{tabular}{p{11.25cm}}
журналист{\tiny noun} корреспондент{\tiny noun} коллега{\tiny noun} порекомендовать{\tiny verb} однокурсник{\tiny noun} зорин{\tiny noun} минаев{\tiny noun} звукооператор{\tiny noun} доценко{\tiny noun} веселов{\tiny noun} фарбер{\tiny noun} бомштейн{\tiny noun};
игорь{\tiny noun} селезнев{\tiny noun}
\\
\hline
земля{\tiny noun} царство{\tiny noun} предание{\tiny noun} владычество{\tiny noun} владетель{\tiny noun} издревле{\tiny adv} доныне{\tiny adv} чертог{\tiny noun};
царь{\tiny noun} кой{\tiny det} обычай{\tiny noun} знатный{\tiny adj} местопребывание{\tiny noun}
\\
\end{tabular}\\
\hline
\begin{center}6\end{center} &
\begin{tabular}{p{11.25cm}}
слово{\tiny noun} речь{\tiny noun} смысл{\tiny noun} вполне{\tiny adv} представление{\tiny noun} понятие{\tiny noun} выражение{\tiny noun} сущность{\tiny noun} действительность{\tiny noun} несомненно{\tiny adv} рассуждение{\tiny noun} суждение{\tiny noun} несомненный{\tiny adj};
именно{\tiny part} характер{\tiny noun}
\\
\hline
отправляться{\tiny verb} отправлять{\tiny verb} прибывать{\tiny verb} направляться{\tiny verb} добираться{\tiny verb} перебираться{\tiny verb} перевозить{\tiny verb} вывозить{\tiny verb} отбывать{\tiny verb} эвакуировать{\tiny verb} прилетать{\tiny verb} переправлять{\tiny verb} эвакуироваться{\tiny verb} угнать{\tiny verb} увозить{\tiny verb}
\\
\end{tabular}\\
\hline
\begin{center}7\end{center} &
\begin{tabular}{p{11.25cm}}
best{\tiny noun} store{\tiny noun} original{\tiny noun} fair{\tiny noun} week{\tiny noun} of::the{\tiny noun} rebel{\tiny noun} trinity{\tiny noun} harmony{\tiny noun} sales{\tiny noun} different{\tiny noun} traveller{\tiny noun} creator{\tiny noun} celebrity{\tiny noun} mystic{\tiny noun}
\\
\hline
удаваться{\tiny verb} попытаться{\tiny verb};
валя{\tiny noun} валер{\tiny noun} сарафанов{\tiny noun};
укол{\tiny noun} барабанный::перепонка{\tiny noun} тромб{\tiny noun};
капилляр{\tiny noun} пыльцевой{\tiny adj};
амбарцумян{\tiny noun} мкртчян{\tiny noun}
\\
\end{tabular}\\
\hline
\end{tabular}

